Personalized Autonomous Driving with Large Language Models: Field Experiments

Integrating large language models (LLMs) in autonomous vehicles enables conversation with AI systems to drive the vehicle. However, it also emphasizes the requirement for such systems to comprehend commands accurately and achieve higher-level personalization to adapt to the preferences of drivers or passengers over a more extended period. In this paper, we introduce an LLM-based framework, Talk2Drive, capable of translating natural verbal commands into executable controls and learning to satisfy personal preferences for safety, efficiency, and comfort with a proposed memory module. This is the first-of-its-kind multi-scenario field experiment that deploys LLMs on a real-world autonomous vehicle. Experiments showcase that the proposed system can comprehend human intentions at different intuition levels, ranging from direct commands like "can you drive faster" to indirect commands like "I am really in a hurry now". Additionally, we use the takeover rate to quantify the trust of human drivers in the LLM-based autonomous driving system, where Talk2Drive significantly reduces the takeover rate in highway, intersection, and parking scenarios. We also validate that the proposed memory module considers personalized preferences and further reduces the takeover rate by up to 65.2% compared with those without a memory module. The experiment video can be watched at https://www.youtube.com/watch?v=4BWsfPaq1Ro

==> tables/main_result_table.tex <==
\begin{table*}[!t]
\centering
\caption{Talk2Drive Performance Outcome with Various LLM Models and Command Categories}
%\caption{Talk2Drive Performance Outcome with Various LLM Models and Command Categories. It details the evaluation metrics resulting from processing commands with varying levels of directness across different driver types. The table captures the framework's ability to interpret and execute drivers' commands, reflecting the variations in command response times and vehicle dynamics for each LLM model.}
\begin{tabular}{cccccccc} 
    \Xhline{1pt}
        %\begin{tabular}[c]{@{}c@{}}Driver\\Type\end{tabular} &
        Driver Type &
        LLM Model &
        \begin{tabular}[c]{@{}c@{}}Level of\\Directness\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}LLM\\Latency(s)\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Average\\LLM Latancy(s)\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Actual\\Speed Difference\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Speed\\Variance\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Mean Absolute\\Acceleration($m \cdot s^{-2}$)\end{tabular}  \\ 
    \Xhline{1pt}
   % \multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Driver Type\\A\end{tabular}} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & \uppercase\expandafter{\romannumeral1}& 2.6 & \multirow{3}{*}{2.3} & +94.9\% & 0.82 & 1.7 \\
   \multirow{12}{*}{Aggresive} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & \uppercase\expandafter{\romannumeral1}& 2.6 & \multirow{3}{*}{2.3} & +94.9\% & 0.82 & 0.18 \\
    & & \uppercase\expandafter{\romannumeral2}& 2.3 & & +61.1\% & 0.32 & 0.14 \\
    & & \uppercase\expandafter{\romannumeral3}& 1.9 & & +96.1\% & 0.84 & 0.18 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 6.8 & \multirow{3}{*}{7.2} & +91.5\% & 0.90 & 0.14 \\
    & & \uppercase\expandafter{\romannumeral2}& 7.3 & & +59.7\% & 0.34 & 0.15 \\
    & & \uppercase\expandafter{\romannumeral3}& 7.5 & & +90.0\% & 0.94 & 0.16 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}} & \uppercase\expandafter{\romannumeral1}& 2.5 & \multirow{3}{*}{2.9} & +97.0\% & 0.81 & 0.16 \\
    & & \uppercase\expandafter{\romannumeral2}& 2.6 & & +62.0\% & 0.29 & 0.13 \\
    & & \uppercase\expandafter{\romannumeral3}& 3.5 & & +94.8\% & 0.85 & 0.17 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 2.3 & \multirow{3}{*}{1.8} & +93.0\% & 0.90 & 0.17 \\
    & & \uppercase\expandafter{\romannumeral2}& 1.6 & & +61.4\% & 0.30 & 0.13 \\
    & & \uppercase\expandafter{\romannumeral3}& 1.6 & & +61.1\% & 0.27 & 0.13 \\ 
    \Xhline{1pt}
    %\multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Type\\B\end{tabular}} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & \uppercase\expandafter{\romannumeral1}& 2.6 & \multirow{3}{*}{2.4} & +22.8\% & 0.08 & 1.3 \\
    \multirow{12}{*}{Moderate} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & \uppercase\expandafter{\romannumeral1}& 2.6 & \multirow{3}{*}{2.4} & +22.8\% & 0.08 & 0.10 \\
    & & \uppercase\expandafter{\romannumeral2}& 2.0 & & +35.5\% & 0.12 & 0.11 \\
    & & \uppercase\expandafter{\romannumeral3}& 2.5 & & +35.5\% & 0.12 & 0.11 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 5.1 & \multirow{3}{*}{6.3} & +10.5\% & 0.06 & 0.09 \\
    & & \uppercase\expandafter{\romannumeral2}& 7.4 & & +56.8\% & 0.42 & 0.08 \\
    & & \uppercase\expandafter{\romannumeral3}& 6.4 & & -38.5\% & 0.10 & 0.15 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}} & \uppercase\expandafter{\romannumeral1}& 2.7 & \multirow{3}{*}{3.0} & +23.1\% & 0.08 & 0.10 \\
    & & \uppercase\expandafter{\romannumeral2}& 2.4 & & +35.0\% & 0.12 & 0.11 \\
    & & \uppercase\expandafter{\romannumeral3}& 3.8 & & +35.7\% & 0.12 & 0.12 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 2.2 & \multirow{3}{*}{1.9} & +35.3\% & 0.11 & 0.11 \\
    & & \uppercase\expandafter{\romannumeral2}& 1.5 & & +24.6\% & 0.08 & 0.09 \\
    & & \uppercase\expandafter{\romannumeral3}& 1.9 & & +35.6\% & 0.12 & 0.01 \\ 
    \Xhline{1pt}
    \multirow{12}{*}{Conservative} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & \uppercase\expandafter{\romannumeral1}& 2.9 & \multirow{3}{*}{5.2} & -53.5\% & 0.09 & 0.05 \\
    & & \uppercase\expandafter{\romannumeral2}& 10.9 & & +0.0\% & 0.05 & 0.07 \\
    & & \uppercase\expandafter{\romannumeral3}& 1.9 & & +0.1\% & 0.05 & 0.07 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 6.7 & \multirow{3}{*}{7.0} & -53.4\% & 0.10 & 0.05 \\
    & & \uppercase\expandafter{\romannumeral2}& 6.4 & & -53.3\% & 0.10 & 0.05 \\
    & & \uppercase\expandafter{\romannumeral3}& 8.0 & & -80.3\% & 0.10 & 0.07 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}} & \uppercase\expandafter{\romannumeral1}& 3.0 & \multirow{3}{*}{2.5} & -54.0\% & 0.09 & 0.05 \\
    & & \uppercase\expandafter{\romannumeral2}& 2.2 & & -28.7\% & 0.09 & 0.06 \\
    & & \uppercase\expandafter{\romannumeral3}& 2.3 & & -53.8\% & 0.09 & 0.05 \\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}} & \uppercase\expandafter{\romannumeral1}& 1.6 & \multirow{3}{*}{1.6} & -53.8\% & 0.10 & 0.05 \\
    & & \uppercase\expandafter{\romannumeral2}& 1.9 & & -27.7\% & 0.09 & 0.06 \\
    & & \uppercase\expandafter{\romannumeral3}& 1.4 & & -54.3\% & 0.08 & 0.05 \\ 
    \Xhline{1pt}
    No Human Input & (without LLM) & & & & & 0.05 & 0.07 \\ 
    \Xhline{1pt}
    & & & & & & & \\
    & & & & & & & \\
    & & & & & & & \\
    & & & & & & & \\
    & & & & & & & \\
    & & & & & & &
\end{tabular}
\label{tab:mainresult}
\end{table*}

==> tables/main_result_table_old.tex <==
\begin{table*}[ht!]
\centering
\caption{Talk2Drive Performance with Different LLM Models and Various Command Types}
\begin{tabular}{cccccccc} 
    \Xhline{1pt}
        \begin{tabular}[c]{@{}c@{}}Command\\Category\end{tabular} &
        LLM Model &
        \begin{tabular}[c]{@{}c@{}}Level of\\Directness\end{tabular} &
        LLM Latency (s) &
        \begin{tabular}[c]{@{}c@{}}Mean\\LLM Latancy (s)\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Speed Difference\end{tabular} &
        Speed Variance&
        \begin{tabular}[c]{@{}c@{}}Mean\\Jerk\end{tabular} \\ 
    \Xhline{1pt}
    \multirow{12}{*}{Fastest} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & 1 & 2.5773 & \multirow{3}{*}{2.2649} & +94.88\% & 10.5856 & ...\\
    & & 2 & 2.2757 &   & +61.06\% & 4.2099    & ...\\
    & & 3 & 1.9417 &   & +96.10\% & 10.8803   & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & 1 & 6.7961 & \multirow{3}{*}{7.1918} & +91.54\% & 11.7159 & ...\\
    & & 2 & 7.2745 &   & +59.69\% & 4.4508    & ...\\
    & & 3 & 7.5048 &   & +89.99\% & 12.2404   & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}}    & 1 & 2.4768 & \multirow{3}{*}{2.8598} & +96.95\% & 10.4861 & ...\\
    & & 2 & 2.5673 &   & +61.97\% & 3.7967    & ...\\
    & & 3 & 3.5353 &   & +94.77\% & 10.9909   & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}}    & 1 & 2.2871 & \multirow{3}{*}{1.8395} & +92.99\% & 11.6617 & ...\\
    & & 2 & 1.599  &   & +61.39\% & 3.8700    & ...\\
    & & 3 & 1.6325 &   & +61.12\% & 3.5629    & ...\\ 
    \Xhline{1pt}
    \multirow{12}{*}{\begin{tabular}[c]{@{}c@{}}Slightly\\Faster\end{tabular}} & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}} & 1 & 2.5575 & \multirow{3}{*}{2.3623} & +22.83\% & 1.0220 & ...\\
    & & 2 & 2.0062 &   & +35.46\% & 1.5248    & ...\\
    & & 3 & 2.5232 &   & +35.54\% & 1.6099    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & 1 & 5.1203 & \multirow{3}{*}{6.3164} & +10.46\% & 0.7869 & ...\\
    & & 2 & 7.4005 &   & +56.76\% & 5.4124    & ...\\
    & & 3 & 6.4285 &   & -38.48\% & 1.3482    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}}    & 1 & 2.6932 & \multirow{3}{*}{2.9866}  & +23.08\% & 1.0000 & ...\\
    & & 2 & 2.4285 &   & +34.99\% & 1.5155    & ...\\
    & & 3 & 3.8381 &   & +35.67\% & 1.5983    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}}    & 1 & 2.1876 & \multirow{3}{*}{1.8726}  & +35.31\% & 1.4858 & ...\\
    & & 2 & 1.4906 &   & +24.63\% & 1.0066    & ...\\
    & & 3 & 1.9397 &   & +35.61\% & 1.5474    & ...\\ 
    \Xhline{1pt}
    \multirow{12}{*}{Slower}               & \multirow{3}{*}{PaLM 2~\cite{anil_palm_2023}}   & 1 & 2.9151 & \multirow{3}{*}{5.2373}  & -53.49\% & 1.2265 & ...\\
    & & 2 & 10.9035     &   & +0.02\%  & 0.6523    & ...\\
    & & 3 & 1.8934 &   & +0.07\%  & 0.6536    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3.5 Turbo~\cite{openai_chatgpt_2023}} & 1 & 6.7194 & \multirow{3}{*}{7.0400}  & -53.37\% & 1.3103 & ...\\
    & & 2 & 6.3831 &   & -53.34\% & 1.3409    & ...\\
    & & 3 & 8.0174 &   & -80.31\% & 1.2656    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-4~\cite{openai_gpt-4_2023}}    & 1 & 2.979  & \multirow{3}{*}{2.4965}  & -54.04\% & 1.1920 & ...\\
    & & 2 & 2.238  &   & -28.70\% & 1.1422    & ...\\
    & & 3 & 2.2726 &   & -53.77\% & 1.1318    & ...\\ 
    \cline{2-8}
    & \multirow{3}{*}{GPT-3~\cite{openai_chatgpt_2023}}    & 1 & 1.625  & \multirow{3}{*}{1.6260}  & -53.80\% & 1.2382 & ...\\
    & & 2 & 1.8859 &   & -27.71\% & 1.1177    & ...\\
    & & 3 & 1.3672 &   & -54.28\% & 1.0753    & ...\\ 
    \Xhline{1pt}
    Baseline & & & & & & 0.660210593 & ...\\
    \Xhline{1pt}
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & & & & & & \\
\end{tabular}
\label{tab:mainresult}
\end{table*}
